Bayesian Inference in Nonparametric Dynamic State-Space Models

We introduce state-space models where the functionals of the observational and the evolutionary equations are unknown, and treated as random functions evolving with time. Thus, our model is nonparametric and generalizes the traditional parametric state-space models. This random function approach also frees us from the restrictive assumption that the functional forms, although time-dependent, are of fixed forms. The traditional approach of assuming known, parametric functional forms is questionable, particularly in state-space models, since the validation of the assumptions require data on both the observed time series and the latent states; however, data on the latter are not available in state-space models. We specify Gaussian processes as priors of the random functions and exploit the "look-up table approach" of \ctn{Bhattacharya07} to efficiently handle the dynamic structure of the model. We consider both univariate and multivariate situations, using the Markov chain Monte Carlo (MCMC) approach for studying the posterior distributions of interest. In the case of challenging multivariate situations we demonstrate that the newly developed Transformation-based MCMC (TMCMC) of \ctn{Dutta11} provides interesting and efficient alternatives to the usual proposal distributions. We illustrate our methods with a challenging multivariate simulated data set, where the true observational and the evolutionary equations are highly non-linear, and treated as unknown. The results we obtain are quite encouraging. Moreover, using our Gaussian process approach we analysed a real data set, which has also been analysed by \ctn{Shumway82} and \ctn{Carlin92} using the linearity assumption. Our analyses show that towards the end of the time series, the linearity assumption of the previous authors breaks down.

==> simstudies_univariate.tex <==

\subsection{Data generated from our univariate, Gaussian process-based model}
\label{subsec:gp_data_generation}

We generate a data set $\{y_t:t=1,\ldots,T+1\}$, where $T=100$, by setting $\beta_{0,f}=0=\beta_{0,g}$,
$\beta_{1,f}=0.01=\beta_{1,g}$, $\beta_{2,f}=0.1=\beta_{2,g}$, $\sigma_f=0.5=\sigma_g$,
$\sigma_{\epsilon}=0.1=\sigma_{\eta}$, and $r_{1,f}=r_{2,f}=r_{1,g}=r_{2,g}=1$. 

In order to simulate the data we need to properly choose the two-dimensional grid $\bG_z$. To this end we 
set $n=100$, and select the first component of $\bG_z$ by generating a random number from each of the intervals
$[i,i+1]$; $i=0,\ldots,99$. We choose the second component by dividing the interval $[-1,1]$
into 100 sub-intervals of equal length and then generating a random number uniformly from each
of the sub-intervals. We simulate $x_0\sim N(0,1)$ (in other words, we set $\mu_{x_0}=0$ and
$\sigma_{x_0}=1$) and $x_1,\ldots,x_{T+1}$, $\bD_z$ using the 
procedure detailed in Section \ref{subsec:lookup_prior_conditionals}. We then simulate 
$\bD_{T+1}\sim N_{T+1}(\bH_{D_{T+1}}\bbeta_f,\sigma^2_f\bA_{f,D_{T+1}}+\sigma^2_{\epsilon}\bI_{T+1})$.  
We set aside the last data point $(x_{T+1},y_{T+1})$ for the purpose of forecasting.

\subsubsection{Choice of prior parameters}
\label{subsubsec:gp_data_prior_choice}

In order to choose the parameters of the log-normal priors of the smoothness parameters, we 
set the mean of the log-normal prior with parameters $\mu$ and $\sigma^2$,
given by $\exp(\mu+\sigma^2/2)$, to 1. This yields $\mu= -\sigma^2/2$. Since the variance
of this log-normal prior is given by $(\exp(\sigma^2)-1)\exp(2\mu+\sigma^2)$, the relation
$\mu=-\sigma^2/2$ implies that the variance is $\exp(\sigma^2)-1=\exp(-2\mu)-1$. We set 
$\sigma^2=1$, so that $\mu=-0.5$. This implies that the mean is 1 and the variance is approximately 2,
for the priors of each smoothness parameter $r_{i,f}$ and $r_{i,g}$; $i=1,2$.

For the choice of the parameters of the priors of $\sigma^2_f$, $\sigma^2_g$, $\sigma^2_{\epsilon}$ 
and $\sigma^2_{\eta}$,
we first note that the mean is of the form $\gamma/(\alpha-2)$ and the variance is of the form
$2\gamma^2/\{(\alpha-2)^2(\alpha-4)\}$. Thus, if we set $\gamma/(\alpha-2)=a$, then the variance becomes
$2a^2/(\alpha-4)$. Here we set $a=0.5,0.5,0.1,0.1$, respectively, for $\sigma^2_f$, $\sigma^2_g$, 
$\sigma^2_{\epsilon}$, 
$\sigma^2_{\eta}$. For each of these priors we set $\alpha=4.01$, so that the variance is of the form
$200a^2$.

We set the priors of $\bbeta_f$ and $\bbeta_g$ to be trivariate normal with zero mean and 
the identity matrix as the variance.

\subsubsection{MCMC implementation}
\label{subsubsec:gp_data_mcmc}

We discarded the first 1000 iterations a burn-in and stored the next 50,000 iterations for inference.
For simulation of $x_0,x_1,\ldots,x_T$, we were able to achieve much better acceptance
rates with random walk proposals with variance 0.1, than with the proposals described 
in Sections \ref{subsubsec:fullcond_x_0} and \ref{subsubsec:fullcond_x_t}.
Also, better acceptance rates were the results of replacing the proposal densities of
$\sigma^2_f$, $\sigma^2_g$, $\sigma^2_{\epsilon}$ and $\sigma^2_{\eta}$ described in Sections 
\ref{subsubsec:fullcond_sigma_f_g} and \ref{subsubsec:fullcond_sigma_e_eta}, respectively,
with normal random walk proposals with variances 0.05. 
For updating the smoothness parameters we used normal random walk proposals with variances 0.005.
To set up the grid $\bG_z$ for the model-fitting purpose, we considered $[-1,1]$ to be a grid space for $x$, which
is the same as the grid space used for simulating the data.
%contains $[-0.33,0.32]$ as a subspace. 
We chose $n=100$ points randomly by selecting a point from each of 100 sub-intervals
of equal length, forming a partition of $[-1,1]$. We chose the first component of the grid (corresponding to the time
component) by uniformly drawing from each subinterval $[i,i+1]$; $i=0,\ldots,99$. %with $h=0.02$.
%In fact, as will be seen subsequently, this time interval seems very adequate for the forecast distributions.
To ascertain the adequacy of the size of the grid $\bG_z$ we experimented by increasing the
size from $n=100$ to $n=200$ and by enlarging the space of the second component of the grid from
$[-1,1]$ to $[-2,2]$, 
but the resultant inference remained almost exactly same, suggesting that
$n=100$ is adequate. 
We could have increased the sampling interval for the time component to include the possibility of interpolation, rather
than extrapolation, for obtaining the forecast distributions. 
%However, this would coarsen the grid and might decrease accuracy
%of the consequent results. 
However, the true forecast values are well-captured by the corresponding posterior (forecast) distributions,
showing that this time interval is adequate for the forecast distributions.
In order to prevent numerical instability of the correlation matrices we added a small positive quantity ($10^{-5}$)
to each diagonal element.
We assessed convergence of our MCMC algorithm using informal diagnostics---there has been no evidence
of non-convergence.
Our implementation of this model took about 15 hours in an ordinary laptop.

\subsubsection{Results of model-fitting}
\label{subsubsec:gp_data_results}

\begin{figure}%[htp]
\centering
  \subfigure{ \label{fig:beta_f_1_simdata}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/beta_f_1-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:beta_f_2_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/beta_f_2-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:beta_f_3_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/beta_f_3-crop.pdf}}\\
  \vspace{2mm}
  \subfigure{ \label{fig:beta_g_1_simdata}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/beta_g_1-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:beta_g_2_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/beta_g_2-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:beta_g_3_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/beta_g_3-crop.pdf}}\\
  \vspace{2mm}
  \subfigure{ \label{fig:sigma_f_simdata}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/sigma_f-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:sigma_g_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/sigma_g-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:sigma_e_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/sigma_e-crop.pdf}}
 \caption{{\bf Simulation study with data generated from the Gaussian process model}: 
 Posterior densities of $\beta_{0,f}$, $\beta_{1,f}$, $\beta_{2,f}$, $\beta_{0,g}$, $\beta_{1,g}$,
 $\beta_{2,g}$, $\sigma_f$, $\sigma_g$, and $\sigma_{\epsilon}$. 
 The solid line stands for the true values of the respective parameters.}
 \label{fig:simdata_rw}
 \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}%[htp]
\centering
  \subfigure{ \label{fig:sigma_eta_simdata}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/sigma_eta-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:r_f_1_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/r_f_1-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:r_f_2_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/r_f_2-crop.pdf}}\\
  \vspace{2mm}
  \subfigure{ \label{fig:r_g_1_simdata}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/r_g_1-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:r_g_2_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/r_g_2-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:x0_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/x0-crop.pdf}}\\
  \vspace{2mm}
  \subfigure{ \label{fig:forecasted_x_simdata}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/forecasted_x-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:forecasted_y_simdata} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_rw/forecasted_y-crop.pdf}}
 \caption{{\bf Simulation study with data generated from the Gaussian process model}: 
 Posterior densities of $\sigma_{\eta}$, $r_{1,f}$, $r_{2,f}$, $r_{1,g}$, $r_{2,g}$,
 $x_0$, $x_{T+1}$ (one-step forecasted $x$), and $y_{T+1}$ (one-step forecasted $y$). 
 The solid line stands for the true values of the respective parameters.}
 \label{fig:simdata_rw2}
 \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}%[htp]
\centering
  \subfigure{ \label{fig:x_time_series_simdata}
   \includegraphics[width=15cm,height=10cm]{plots_simdata_rw/x_time_series-crop.pdf}}
 \caption{{\bf Simulation study with data generated from the Gaussian process model}: 
 95\% highest posterior density credible intervals of the time series $x_1,\ldots,x_T$. 
 The solid line stands for the true time series.}
 \label{fig:simdata_rw3}
 \end{figure}

Figures \ref{fig:simdata_rw}, \ref{fig:simdata_rw2} and \ref{fig:simdata_rw3} show that the true values
of all the unknowns are captured very well by the respective posterior distributions. The forecast
distributions (the posteriors of $x_{101}$ and $y_{101}$) capture their respective true values
particularly well, vindicating the predictive power of our model. The true time series $\{x_1,\ldots,x_{100}\}$
fall well within the lower and the upper 95\% highest posterior density credible limits; however,
increased variability is observed as time increases. This is not unexpected since  
the errors of approximating the unknown functions accumulate with time. 

\subsection{Data generated from a univariate parametric nonstationary growth model}
\label{subsec:cps_data_generation}

Following \ctn{Carlin92} we generate data from the following model:
\begin{align}
x_t&=\alpha x_{t-1}+\beta x_{t-1}/(1+x^2_{t-1})+\gamma\cos(1.2 (t-1))+u_t\label{eq:cps1}\\
y_t&=x^2_t/20+v_t, \ \ \ t=1,\ldots,100,\label{eq:cps2}
\end{align}
where $x_0=0$. Unlike \ctn{Carlin92} who assumed $u_t$ to have $t$-distribution, here we assume
$u_t\sim N(0,\sigma^2_{\epsilon})$ and $v_t\sim N(0,\sigma^2_{\eta})$, independently for all $t$.
We set $\sigma_{\epsilon}=0.1=\sigma_{\eta}$ and fix
the true values of $(\alpha,\beta,\gamma)$ to be $(0.05,0.1,0.2)$, respectively.
We then generated the data set consisting of 101 data points using these true values.
As before, we set aside the last data point for the purpose of forecasting.

\subsubsection{Choice of prior parameters and MCMC implementation}
\label{subsubsec:cps_data_prior_choice}

For this example, we use the same prior structure described in Section \ref{subsubsec:gp_data_prior_choice}.
To set up the grid $\bG_z$ we first note that the entire true time series falls within the space $[-0.33,0.32]$.
We consider a larger space, $[-0.5,0.5]$, and dividing it into 100 sub-intervals of equal length, select
a value randomly from each such sub-interval. This yields values of the second component of the
two-dimensional grid $\bG_z$. For the first component we generate a number uniformly from each of the
100 sub-intervals $[i,i+1]$; $i=0,\ldots,99$. %where $h=0.01$.

As before we discard the first 1000 MCMC iterations as burn-in and store the next 50,000 iterations for 
inference. We used the normal random walk proposal with variance 0.05 for updating $\sigma_f$, $\sigma_g$,
$\sigma_{\epsilon}$ and $\sigma_{\eta}$ and the normal random walk proposal with variance 1 for updating
$\{x_0,x_1,\ldots,x_T\}$. 
Once again, we added $10^{-5}$ to the diagonal elements of the correlation matrices to avoid 
numerical instability. Informal diagnostics indicated good convergence properties of our MCMC algorithm. 
It took around 15 hours in an ordinary laptop to implement this experiment.

\subsubsection{Results of model-fitting}
\label{subsubsec:cps_data_results}

\begin{figure}%[htp]
\centering
  \subfigure{ \label{fig:beta_f_1_simdata_cps}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/beta_f_1-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:beta_f_2_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/beta_f_2-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:beta_f_3_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/beta_f_3-crop.pdf}}\\
  \vspace{2mm}
  \subfigure{ \label{fig:beta_g_1_simdata_cps}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/beta_g_1-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:beta_g_2_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/beta_g_2-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:beta_g_3_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/beta_g_3-crop.pdf}}\\
  \vspace{2mm}
  \subfigure{ \label{fig:sigma_f_simdata_cps}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/sigma_f-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:sigma_g_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/sigma_g-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:sigma_e_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/sigma_e-crop.pdf}}
 \caption{{\bf Simulation study with data generated from the univariate nonstationary growth model
 of CPS}: 
 Posterior densities of $\beta_{0,f}$, $\beta_{1,f}$, $\beta_{2,f}$, $\beta_{0,g}$, $\beta_{1,g}$,
 $\beta_{2,g}$, $\sigma_f$, $\sigma_g$, and $\sigma_{\epsilon}$. 
 The solid line stands for the true values of the respective parameters.}
 \label{fig:simdata_cps}
 \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}%[htp]
\centering
  \subfigure{ \label{fig:sigma_eta_simdata_cps}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/sigma_eta-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:r_f_1_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/r_f_1-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:r_f_2_simdata-cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/r_f_2-crop.pdf}}\\
  \vspace{2mm}
  \subfigure{ \label{fig:r_g_1_simdata_cps}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/r_g_1-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:r_g_2_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/r_g_2-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:x0_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/x0-crop.pdf}}\\
  \vspace{2mm}
  \subfigure{ \label{fig:forecasted_x_simdata_cps}
   \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/forecasted_x-crop.pdf}}
   \hspace{2mm}
  \subfigure{ \label{fig:forecasted_y_simdata_cps} 
  \includegraphics[width=5cm,height=4cm]{plots_simdata_cps/forecasted_y-crop.pdf}}
 \caption{{\bf Simulation study with data generated from the univariate nonstationary
 growth model of CPS}: 
 Posterior densities of $\sigma_{\eta}$, $r_{1,f}$, $r_{2,f}$, $r_{1,g}$, $r_{2,g}$,
 $x_0$, $x_{T+1}$ (one-step forecasted $x$), and $y_{T+1}$ (one-step forecasted $y$). 
 The solid line stands for the true values of the respective parameters.}
 \label{fig:simdata_cps2}
 \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}%[htp]
\centering
  \subfigure{ \label{fig:x_time_series_simdata_cps}
   \includegraphics[width=15cm,height=10cm]{plots_simdata_cps/x_time_series-crop.pdf}}
 \caption{{\bf Simulation study with data generated from the univariate nonstationary
 growth model of CPS}: 
 95\% highest posterior density credible intervals of the time series $x_1,\ldots,x_T$. 
 The solid line stands for the true time series.}
 \label{fig:simdata_cps3}
 \end{figure}

Figures \ref{fig:simdata_cps}, \ref{fig:simdata_cps2} and \ref{fig:simdata_cps3} show 
the posterior distributions of the unknowns. Note that whenever applicable, the true value
is well-captured by the posteriors in question.
As before, the true values of $x_{101}$ and $y_{101}$ are captured very well
by their respective posteriors. The true time series $\{x_1,\ldots,x_{100}\}$ again
fell well within the lower and the upper 95\% highest posterior density credible limits.
The true values of $\sigma_{\epsilon}$, $\sigma_{\eta}$ and $x_0$ also fell well within
the highest density regions of their respective posterior distributions.
That our Gaussian process approach fits the data so well despite the fact that the
functions $f(\cdot,\cdot)$ and $g(\cdot,\cdot)$ are highly non-linear, is very encouraging.




